Asymmetric Stream Allocation and Linear Decodability in MIMO Coded Caching

Coded caching (CC) can transform cache memory at network devices into an active communication resource and significantly enhance the Degrees of Freedom (DoF) of multi-input multi-output (MIMO) systems by jointly exploiting global caching and spatial multiplexing gains. Existing linearly decodable MIMO-CC designs, however, largely rely on symmetric stream allocation, where all scheduled users receive the same number of streams, which induces coarse DoF granularity and may leave spatial dimensions unused. This letter studies one-shot linearly decodable MIMO-CC delivery with arbitrary per-user stream allocations. We derive a sufficient stream-count decodability condition, expressed through per-user stream counts and multicast-codeword multiplicities, that generalizes the symmetric common-stream feasibility rule. Building on this condition, we develop a greedy multicast scheduling procedure with certified linear decodability, which redistributes coded multicast messages across transmission intervals to realize asymmetric stream allocations. Numerical results show that the proposed scheduler fills DoF-granularity gaps and improves finite-SNR symmetric rates over the state of the art.

==> Figs/data_L11_G8.tex <==
SNR		RsymproposedL11G8t0omg11DoF11					RsymproposedL11G8t2omg4DoF12				RsymproposedL11G8t2omg4DoF15				RsymproposedL11G8t2omg4DoF18				RsymproposedL11G8t2omg4DoF21					RsymproposedL11G8t2omg4DoF24					RsymproposedL11G8t2omg4DoF27				RsymproposedL11G8t2omg4DoF30	
																																		
0			18.4554510658181					29.10577836				30.16767547				30.26369657				30.19260516					30.2135327					27.6532				26.49412924
5			33.3799691861168					47.85780528				51.98309189				54.04792266				54.26628798					54.39852082					50.6997				47.02605108
10			51.5375109535440					68.7746908				77.40996423				83.34790837				86.21486495					87.34880343					83.2867				75.87882707
15			71.0902703161183					90.51270192				104.3411699				115.1625351				122.2513053					127.4143168					124.131				112.5888229
20			91.1578635866648					112.5273168				131.7765426				147.9212902				160.0199879					169.9957654					170.046				156.2191983
25			111.329167250455					134.5870387				159.378676				180.9701078				198.6870484					213.8567177					218.2483				205.1934144
30			131.531300753087					156.6512301				186.927976				214.0493744				237.3206966					257.7548711					267.261				257.7457551

